Large solutions for fractional Laplacian operators

The thesis studies linear and semilinear Dirichlet problems driven by different fractional Laplacians. The boundary data can be smooth functions or also Radon measures. The goal is to classify the solutions which have a singularity on the boundary of the prescribed domain. We first remark the existence of a large class of harmonic functions with a boundary blow-up and we characterize them in terms of a new notion of degenerate boundary trace. Via some integration by parts formula, we then provide a weak theory of Stampacchia's sort to extend the linear theory to a setting including these functions: we study the classical questions of existence, uniqueness, continuous dependence on the data, regularity and asymptotic behaviour at the boundary. Afterwards we develop the theory of semilinear problems, by adapting and generalizing some sub- and supersolution methods. This allows us to build the fractional counterpart of large solutions in the elliptic PDE theory of nonlinear equations, giving sufficient conditions for the existence. The thesis is concluded with the definition and the study of a notion of nonlocal directional curvatures.

==> 1frontespizio.tex <==
\begin{titlepage}

\begin{minipage}{.48\textwidth}
\begin{center}
\includegraphics[width=26mm]{logoUPJV}\\
\textsc{Universit\'e de Picardie Jules Verne}\\
{\it Ecole Doctorale Sciences, Technologie et Sant\'e}
\end{center}
\end{minipage}
\begin{minipage}{.48\textwidth}
\begin{center}
\includegraphics[width=30mm]{logonuovo}\\
\textsc{Universit\`a degli Studi di Milano}\\
{\it Scuola di Dottorato di ricerca in Matematica}
\end{center}
\end{minipage}

\vspace{\stretch{3}}

\begin{center}
{\Huge\bf Th\`ese de Doctorat}
\bigskip

{\bf\itshape\large Sp\'ecialit\'e Mathematiques}
\end{center}

\vspace{\stretch{1}}

\begin{center}

{\large pr\'esent\'ee \`a} 
\bigskip

{\huge\bf l'Universit\'e de Picardie Jules Verne}
\bigskip

{\large par}
\bigskip

{\Huge Nicola Abatangelo}
\bigskip
 
{\large pour obtenir le grade de Docteur de l'Universit\'e de Picardie Jules Verne\\
et le grade de Dottore de l'Universit\`a degli Studi di Milano}

\vspace{\stretch{3}}

{\textbf{\scshape{\huge{\textit{Large Solutions for Fractional \\
\vspace{0.3cm}
Laplacian Operators}}}}}

\vspace{\stretch{6}}

{\large\bf Soutenue le 28 
Septembre 2015, apr\`es avis des rapporteurs, devant le jury d'examen~:
\medskip

\begin{minipage}{.9\textwidth}\large
M. C. Imbert, Directeur de Recherche 
\hfill Rapporteur \\
M. J. L. V\'azquez, Professeur 
\hfill Rapporteur \\
M. A. Farina, Professeur 
\hfill Examinateur \\
M. K. R. Payne, Professeur 
\hfill Examinateur \\
M. L. Dupaigne, Ma\^{i}tre de Conf\'erences \hfill Directeur de Th\`ese\\
M. E. Valdinoci, Professeur \hfill Directeur de Th\`ese \\
M. O. Goubet, Professeur 
\hfill Membre invit\'e \\

\end{minipage}}

\vspace{\stretch{2}}

\begin{minipage}{.48\textwidth}
\includegraphics[width=26mm]{region-picardie}
\end{minipage}
\begin{minipage}{.48\textwidth}
\begin{flushright}
\includegraphics[width=30mm]{loglamfa}
\end{flushright}
\end{minipage}

\end{center}

\end{titlepage}

\thispagestyle{empty}

% ==============================================================================================

\begin{titlepage}

\begin{minipage}{.48\textwidth}
\begin{center}
\includegraphics[width=26mm]{logoUPJV}\\
\textsc{Universit\'e de Picardie Jules Verne}\\
{\it Ecole Doctorale Sciences, Technologie et Sant\'e}
\end{center}
\end{minipage}
\begin{minipage}{.48\textwidth}
\begin{center}
\includegraphics[width=30mm]{logonuovo}\\
\textsc{Universit\`a degli Studi di Milano}\\
{\it Scuola di Dottorato di ricerca in Matematica}
\end{center}
\end{minipage}

\vspace{\stretch{.75}}

\begin{center}
{\large\sc dipartimento di matematica \\

corso di dottorato in matematica, xxviii ciclo}

\vspace{\stretch{2}}

{\Huge\bf Large Solutions for Fractional Laplacian Operators}

\vspace{\stretch{2}}

\large

\hfill Tesi di Dottorato di:

\hfill Nicola Abatangelo

\vspace{\stretch{1}}

\begin{flushleft}
Direttori di tesi: \\
Prof. Enrico Valdinoci, {\small Universit\`a degli Studi di Milano} \\
Prof. Louis Dupaigne, {\small Universit\'e Claude Bernard -- Lyon 1 (Lione, Francia)}

\vspace{\stretch{0.5}}

Coordinatore del corso di dottorato: \\
Prof. Lambertus Van Geemen, {\small Universit\`a degli Studi di Milano}
\end{flushleft}

\vspace{\stretch{1}}

A.A. 2014--2015

\end{center}

\end{titlepage}

\thispagestyle{empty}

